Exploring the Steiner-Soddy Porism

We explore properties and loci of a Poncelet family of polygons -- called here Steiner-Soddy -- whose vertices are centers of circles in the Steiner porism, including conserved quantities, loci, and its relationship to other Poncelet families.

==> 000_setup.tex <==
% https://robjhyndman.com/hyndsight/squeezing-space-with-latex/
\usepackage{mathptmx}
\usepackage{enumitem}
\usepackage{multirow}
%\usepackage{titlesec}
%\titleformat{\section}
%{\normalfont\bfseries}
%{\thesection.}{0.5em}{}
%\usepackage{enumerate}
\usepackage{graphics}
\usepackage{thmtools}
\usepackage{wasysym}
%\usepackage{arxiv}
%\usepackage{enseign}
%\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts

\usepackage{amsthm}
\usepackage{amsbsy,amsmath,amssymb,amscd,amsfonts,float}
\usepackage[pagebackref=true]{hyperref}
\usepackage[nameinlink,capitalize,noabbrev]{cleveref}
%\usepackage{hyperref}
%\usepackage{url}            % simple URL typesetting
%\usepackage{booktabs}       % professional-quality tables
%\usepackage{nicefrac}       % compact symbols for 1/2, etc.
%\usepackage{microtype}      % microtypography

\usepackage{graphicx,float,latexsym,color}
%\usepackage{mathspec}
\usepackage[font={scriptsize,it}]{caption}
\usepackage{subcaption}
\usepackage[export]{adjustbox}
%\let\proof\relax
%\let\endproof\relax

\usepackage{makecell}
\renewcommand{\arraystretch}{1.2}

\usepackage[dvipsnames]{xcolor}

\newtheorem{theorem}{Theorem}
\newtheorem*{theorem*}{Theorem}
\newtheorem{observation}{Observation}
\newtheorem{proposition}{Proposition}
\newtheorem{conjecture}{Conjecture}
\newtheorem{corollary}{Corollary}
\newtheorem{lemma}{Lemma}
\theoremstyle{remark}
\newtheorem{remark}{Remark}
\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{question}{Question}
\hypersetup{
    %bookmarks=true,         % show bookmarks bar?
    %unicode=true,          % non-Latin characters in Acrobat’s bookmarks
    pdftoolbar=true,        % show Acrobat’s toolbar?
    pdfmenubar=true,        % show Acrobat’s menu?
    pdffitwindow=false,     % window fit to page when opened
    pdfstartview={FitH},    % fits the width of 
    colorlinks=true,       % false: boxed links; true: colored links
    linkcolor=OliveGreen,          % color of internal links (change box color with linkbordercolor)
    citecolor=blue,        % color of links to bibliography
    filecolor=black,      % color of file links
    urlcolor=red           % color of external links
}

\usepackage{lineno}
\def\linenumberfont{\normalfont\small\sffamily}
%a4: 210 x 297
%\textwidth=125mm
%\textheight=195mm
\arraycolsep=2pt
\captionsetup{width=120mm}

 \newcommand{\Mod}[1]{\ (\mathrm{mod}\ #1)}
 
\usepackage{comment}
\usepackage{microtype}
\usepackage{footnote}
%\usepackage{tablefootnote}
%\usepackage{longtable}

%\usepackage{night}
\renewcommand{\H}{\mathcal{H}}
\newcommand{\B}{\mathcal{B}}
\renewcommand{\S}{\mathcal{S}}
\newcommand{\Z}{\mathcal{Z}}
\newcommand{\E}{\mathcal{E}}
\newcommand{\T}{\mathcal{T}}
\newcommand{\C}{\mathcal{C}}
\newcommand{\F}{\mathcal{F}}
\renewcommand{\L}{\mathcal{L}}
\renewcommand{\P}{\mathcal{P}}
\newcommand{\D}{\mathbb{D}}
\renewcommand{\T}{\mathbb{T}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Cp}{\mathbb{C}}
\newcommand{\ol}{\overline}
\renewcommand{\l}{\lambda}
\newcommand{\X}{\mathcal{X}}
\newcommand{\Y}{\mathcal{Y}}
\renewcommand{\H}{\mathcal{H}}
%\renewcommand{\Z}{\mathcal{Z}}
\newcommand{\torp}[2]{\texorpdfstring{#1}{#2}}
\newcommand{\ab}{_{\alpha,\beta}}

%\input{000_refcheck}
% https://robjhyndman.com/hyndsight/squeezing-space-with-latex/
\setlength{\abovecaptionskip}{5 pt}
\setlength{\belowcaptionskip}{0pt}
\setlength{\parskip}{0em}
\setlength{\parindent}{1em}
\setlength{\textfloatsep}{0.5 em}
\usepackage[compact]{titlesec}
\titleformat{name=\section}{}{\thetitle.}{1em}{\centering\scshape}
\titleformat{name=\subsection}[runin]{}{\thetitle.}{0em}{\bfseries}
\titlespacing{\section}{0pc}{1.5ex plus .1ex minus .2ex}{0pc}

%\titlespacing{\subsection}{0pc}{1.5ex plus .1ex minus .2ex}{0pc}
\titlespacing{\subsection}{0pc}{0.5pc}{0.5em}

\crefname{conjecture}{Conjecture}{Conjectures}
\crefname{definition}{Definition}{Definitions}

\newcommand{\rulesep}{\unskip\ \vrule\ }
\usepackage{esvect}


%\input{999_refcheck}

==> 001_setup.tex <==
\RequirePackage[fleqn]{amsmath}
% https://robjhyndman.com/hyndsight/squeezing-space-with-latex/
\usepackage{graphicx}
\usepackage[nameinlink,capitalize,noabbrev]{cleveref}
%\usepackage{enumitem}
\usepackage{xcolor}
\usepackage[export]{adjustbox}
\usepackage[font={small}]{caption}
\usepackage{subcaption}
\usepackage{multirow}
\usepackage{paralist}


\renewcommand{\H}{\mathcal{H}}
\newcommand{\B}{\mathcal{B}}
\renewcommand{\S}{\mathcal{S}}
\newcommand{\Z}{\mathcal{Z}}
\newcommand{\E}{\mathcal{E}}
\newcommand{\T}{\mathcal{T}}
\newcommand{\C}{\mathcal{C}}
\newcommand{\F}{\mathcal{F}}
\renewcommand{\L}{\mathcal{L}}
\renewcommand{\P}{\mathcal{P}}
\newcommand{\D}{\mathbb{D}}
\renewcommand{\T}{\mathbb{T}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Cp}{\mathbb{C}}
\newcommand{\ol}{\overline}
\renewcommand{\l}{\lambda}
\newcommand{\X}{\mathcal{X}}
\newcommand{\Y}{\mathcal{Y}}
\renewcommand{\H}{\mathcal{H}}
%\renewcommand{\Z}{\mathcal{Z}}

\newcommand{\rulesep}{\unskip\ \vrule\ }
\usepackage{esvect}

%\usepackage[compact]{titlesec}
\setlength{\abovecaptionskip}{5 pt}
\setlength{\belowcaptionskip}{0pt}
\setlength{\parskip}{0em}
\setlength{\parindent}{1em}
\setlength{\textfloatsep}{0.5 em}

\makeatletter
\let\origsection\section
\renewcommand\section{\@ifstar{\starsection}{\nostarsection}}

\newcommand\nostarsection[1]
{\sectionprelude\origsection{#1}\sectionpostlude}
\newcommand\starsection[1]
{\sectionprelude\origsection*{#1}\sectionpostlude}
\newcommand\sectionprelude{%
  \vspace{-.5em}
}
\newcommand\sectionpostlude{%
  \vspace{-.5em}
}

\makeatother

%\input{999_refcheck}

==> 005_abstract.tex <==
\begin{abstract}
We explore the dynamic geometry of of a Poncelet family of polygons -- called here Steiner-Soddy -- whose vertices are centers of circles in the Steiner porism, closely-related to harmonic polygons. We derive properties specific to when said polygons are triangles, and describe loci of some of its triangle centers.
\vskip .2cm
\keywords{Keywords} triangle, conic, porism, Soddy, Steiner, invariant, conservation.
\vskip .2cm
\noindent \textbf{MSC} {51M04
\and 51N20 \and 51N35\and 68T20}
\end{abstract}


==> 999_outline.tex <==
\subsection{resultados para qualquer N}

\begin{enumerate}
\item considerar a familia P q é imagem polar dos poligonos harmonicos
com respeito ao circumcirculo
\item corolario: esta familia esta inscrita numa conica e circumscreve um circulo
\item qdo o circumcentro esta sobre um co-vertice da inellipse de Brocard B,
a familia esta inscrita numa parabola
\item familia conserva soma de meias tangentes
\end{enumerate}


\subsection{caso N=3}

\begin{enumerate}
\item familia "Steiner-Soddy" sao os tangenciais do porisma de Brocard, i.e., sua imagem polar com respeito ao circumcirculo. 
\item é ponceletiana, i.e., inscrita numa conica.
\item foci da conica externa sao X176 e X175, os centros dos circulos de Soddy
\item conserva soma de tan(t/2). qdo esta soma é igual a 2, o circulo externo de soddy é uma reta, paralela a diretriz. Mencionar resulatdo do Hajja e Yff.
\item qdo o aspect ratio de B é $\phi/2$, a familia esta inscrita numa parabola.
\item a soma de meias tangentes tem q ser ajustada a ter sinal dependendo do ramo da hiperbole q os vertices do tangencial se encontram.
\item Zaslavsky: conservacoes genericas para qq familia inscrita em parabola e circumscrevendo circulo
\end{enumerate}

\subsection{N=3 Loci}

Quando a familia esta inscrita numa parabola:

\begin{itemize}
\item ha um aspect ratio da B (em torno de 1.225) onde o locus do X4 é a hiperbole externa da familia.
\item o locus de X4 é uma reta paralela a diretriz.
    o locus de X4 é sempre uma reta paralela a diretriz para q familia inscrita numa parabola e circumscrevendo um circulo cujo centro esta no eixo
    \item falar da familia inscrita numa parabola e circumscrevendo circulo, contendo um equilatero.
    \item X20 parado para todas elas
    \item citar paper com Bellio (imagem polar do bicentrico q conserva soma de duplos senos)
\end{itemize}



\begin{enumerate}
\item se um triangulo de referencia é agudo, seu X3 (resp. X6) coincide com o X1 (resp. X7) do tangencial. corolario: enquanto o de referencia é agudo, X1 e X7 do tangencial estao parados. de outra maneira, o tangencial esta evertido, e X1 e X7 traçam arcos (de alguma curva).
\item X2,3,4,5 (previsto) sao conicas.
\item X6 (nao previsto pela teoria) é uma conica. Para um determinado a/b de B ela passa pelos dois focos de B (a/b=1.053)
\item X8,9,10 sao conicas nao previstas
\item X13,14,15,16 sao circulos
\item ponto de de Longchamps se move num segmento (elipse com eixo menor = 0?)
\item X65 pode ser circulo (enquanto o ref. é agudo)
\item X77, X170 são segmentos
\item X80 circulo
\item X105 é circulo tangente a elipse externa e  tem o centro no eixo da elipse!
\item X175 e X176 sao os focos da conica externa, se a/b < phi/2 (ou seja, conica externa é uma elipse)
\end{enumerate}




==> 999_refcheck.tex <==
\usepackage{refcheck}
% make refcheck work w cref
% https://tex.stackexchange.com/questions/87610/making-refcheck-work-with-cleveref
\makeatletter
\newcommand{\refcheckize}[1]{%
  \expandafter\let\csname @@\string#1\endcsname#1%
  \expandafter\DeclareRobustCommand\csname relax\string#1\endcsname[1]{%
    \csname @@\string#1\endcsname{##1}\@for\@temp:=##1\do{\wrtusdrf{\@temp}\wrtusdrf{{\@temp}}}}%
  \expandafter\let\expandafter#1\csname relax\string#1\endcsname
}
\newcommand{\refcheckizetwo}[1]{%
  \expandafter\let\csname @@\string#1\endcsname#1%
  \expandafter\DeclareRobustCommand\csname relax\string#1\endcsname[2]{%
    \csname @@\string#1\endcsname{##1}{##2}\wrtusdrf{##1}\wrtusdrf{{##1}}\wrtusdrf{##2}\wrtusdrf{{##2}}}%
  \expandafter\let\expandafter#1\csname relax\string#1\endcsname
}
\makeatother

\refcheckize{\cref}
\refcheckize{\Cref}
\refcheckizetwo{\crefrange}
\refcheckizetwo{\Crefrange}

==> overflow.tex <==
Since inversions send circles to circle, the pairwise contacts between circles in the chain are concyclic. Interestingly, these are the vertices\footnote{In fact, the tangency points of circles in the chain with either the inner or outer Soddy circles are vertices of 2 other harmonic polygons.} of a {\em harmonic polygon} (shown magenta in \cref{fig:intro-n5}), namely, one which is circle-inscribed and contains a special point $K$ known as the {\em symmedian point} \cite{casey1888} such that the distance to each side is at a constant proportion to the sidelength, see \cref{fig:intro-n5}. Over the Steiner porism, said harmonic polygons are a circle-inscribed Poncelet porism circumscribing a caustic known as the {\em Brocard inellipse}. It has been recently shown that the HF conserves the sum the cotangents of its internal angles, as well as other related functions \cite{roitman2021-harmonic}.
